Studying excited-state-specific perturbation theory on the Thiel set

We explore the performance of a recently-introduced $N^5$-scaling excited-state-specific second order perturbation theory (ESMP2) on the singlet excitations of the Thiel benchmarking set. We find that, without regularization, ESMP2 is quite sensitive to $\pi$ system size, performing well in molecules with small $\pi$ systems but poorly in those with larger $\pi$ systems. With regularization, ESMP2 is far less sensitive to $\pi$ system size and shows a higher overall accuracy on the Thiel set than CC2, EOM-CCSD, CC3, and a wide variety of time-dependent density functional approaches. Unsurprisingly, even regularized ESMP2 is less accurate than multi-reference perturbation theory on this test set, which can in part be explained by the set's inclusion of some doubly excited states but none of the strong charge transfer states that often pose challenges for state-averaging. Beyond energetics, we find that the ESMP2 doubles norm offers a relatively low-cost way to test for doubly excited character without the need to define an active space.

==> CI_amps/acetamide_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetamide_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for acetamide.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$2(0.58) & H$-$1$\rightarrow$L$+$2(0.85) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$5(0.27) & H$-$1$\rightarrow$L$+$5(0.37) \\ 
\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(-0.60) & H$\rightarrow$L$+$2(-0.70) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L(-0.50) \\ 
\hspace{0.0mm} & & H$\rightarrow$L(-0.23) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$1(-0.21) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$5(0.25) & \\
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/acetone_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetone_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for acetone.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.58) & H$\rightarrow$L$+$1(-0.88) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$4(-0.20) & H$\rightarrow$L$+$4(-0.29) \\ 
\hspace{0.0mm} & H$-$7$\rightarrow$L$+$1(0.20) & \\ 
\hspace{0.0mm} $1^1B_{1}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$1(-0.41) & H$-$3$\rightarrow$L$+$1(-0.74) \\ 
\hspace{0.0mm} & H$-$6$\rightarrow$L$+$1(-0.41) & H$-$6$\rightarrow$L$+$1(-0.48) \\ 
\hspace{0.0mm} & H$-$8$\rightarrow$L$+$1(0.23) & H$-$3$\rightarrow$L$+$4(-0.23) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(0.60) & H$\rightarrow$L$+$2(-0.68) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.17) & H$-$1$\rightarrow$L$+$1(-0.58) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/adenine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:adenine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for adenine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.50) & H$\rightarrow$L$+$2(-0.70) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(0.29) & H$-$1$\rightarrow$L(-0.57) \\
\hspace{0.0mm} $3^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.65) & H$\rightarrow$L(-0.88) \\ 
\hspace{0.0mm} & & H$-$2$\rightarrow$L$+$5(-0.27) \\ 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(-0.49) & H$-$2$\rightarrow$L(0.89) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$2(0.33) & H$-$2$\rightarrow$L$+$5(-0.27) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$5(0.23) & \\
\hspace{0.0mm} $2^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$2(0.66) & H$-$2$\rightarrow$L$+$2(0.92) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/benzene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for benzene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2u}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.50) & H$\rightarrow$L$+$1(0.66) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.50) & H$-$1$\rightarrow$L(-0.66) \\ 
\hspace{0.0mm} $1^1B_{1u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.50) & H$-$1$\rightarrow$L$+$1(0.68) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.50) & H$\rightarrow$L(0.68) \\ 
\hspace{0.0mm} $1^1E_{1u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(-0.48) & H$-$1$\rightarrow$L(0.66) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.49) & H$\rightarrow$L$+$1(0.66) \\ 
\hspace{0.0mm} $2^1E_{2g}$ & & \\ 
\hspace{0.0mm} & H$-$4$\rightarrow$L$+$1(0.69) & H$-$4$\rightarrow$L$+$1(0.84) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$9(-0.32) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$1(0.20) \\
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/benzoquinone_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzoquinone_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for benzoquinone.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{u}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(-0.62) & H$-$2$\rightarrow$L(0.89) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$3(-0.24) & H$-$3$\rightarrow$L$+$3(0.26) \\ 
\hspace{0.0mm} $1^1B_{1g}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.59) & H$-$3$\rightarrow$L(-0.90) \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$3(0.27) & H$-$2$\rightarrow$L$+$3(-0.26) \\ 
\hspace{0.0mm} $1^1B_{3g}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.69) & H$-$1$\rightarrow$L(0.95) \\ 
\hspace{0.0mm} $1^1B_{1u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.66) & H$\rightarrow$L(0.93) \\ 
\hspace{0.0mm} $1^1B_{3u}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(-0.61) & H$-$2$\rightarrow$L$+$1(-0.93) \\ 
\hspace{0.0mm} & H$-$0$\rightarrow$L(-0.30) & \\ 
\hspace{0.0mm} $2^1B_{3g}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(-0.67) & H$\rightarrow$L$+$1(-0.93) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/butadiene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:butadiene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for butadiene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.69) & H$\rightarrow$L(-0.95) \\ 
\hspace{0.0mm} $2^1A_{g}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.48) & H$\rightarrow$L$+$4(-0.63) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$4(0.45) & H$-$1$\rightarrow$L(-0.54) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/cyclopentadiene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopentadiene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for cyclopentadiene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.69) & H$\rightarrow$L(-0.96) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.49) & H$-$1$\rightarrow$L(0.67) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$7(0.47) & H$\rightarrow$L$+$7(-0.59) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/cyclopropene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopropene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for cyclopropene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.68) & H$-$1$\rightarrow$L(0.94) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$14(0.21) \\ 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.67) & H$\rightarrow$L(0.93) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/cytosine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cytosine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for cytosine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.66) & H$-$2$\rightarrow$L(0.80) \\ 
\hspace{0.0mm} & & H$-$3$\rightarrow$L(-0.39) \\ 
\hspace{0.0mm} & & H$-$2$\rightarrow$L$+$4(0.28) \\ 
\hspace{0.0mm} $2^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$4(0.44) & H$-$3$\rightarrow$L$+$4(-0.56) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$4(0.41) & H$-$2$\rightarrow$L$+$4(-0.56)\\ 
\hspace{0.0mm} & & H$-$3$\rightarrow$L(-0.43) \\
\hspace{0.0mm} $3^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.60) & H$-$1$\rightarrow$L(0.90) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/ethene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:ethene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for ethene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.69) & H$\rightarrow$L(-0.96) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/formaldehyde_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formaldehyde_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for formaldehyde.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.62) & H$\rightarrow$L(0.91) \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(-0.20) & H$\rightarrow$L$+$5(-0.23) \\ 
\hspace{0.0mm} $1^1B_{1}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.63) & H$-$2$\rightarrow$L(0.91) \\ 
\hspace{0.0mm} & & H$-$2$\rightarrow$L$+$5(-0.24) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(0.60) & H$\rightarrow$L$+$2(0.80) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L(0.41) \\ 
\hspace{0.0mm} & & H$\rightarrow$L(-0.28) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/formamide_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formamide_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for formamide.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L+2(-0.64) & H$-$1$\rightarrow$L$+$2(-0.92) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$6(0.24) \\ 
\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.56) & H$-$1$\rightarrow$L(0.74) \\ 
\hspace{0.0mm} & H$\rightarrow$L+2(-0.25) & H$\rightarrow$L(0.53) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/furan_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:furan_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for furan.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.68) & H$\rightarrow$L(-0.94) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.53) & H$-$1$\rightarrow$L(-0.69) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$5(0.43) & H$\rightarrow$L$+$5(-0.59) \\ 
\hspace{0.0mm} $3^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$5(-0.50) & H$\rightarrow$L$+$5(-0.68) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.45) & H$-$1$\rightarrow$L(0.59) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/hexatriene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:hexatriene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for hexatriene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.68) & H$\rightarrow$L(-0.95) \\ 
\hspace{0.0mm} $2^1A_{g}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.43) & H$-$1$\rightarrow$L(-0.59) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(-0.43) & H$\rightarrow$L$+$2(-0.55) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/imidazole_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:imidazole_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for imidazole.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(-0.56) & H$-$2$\rightarrow$L$+$1(-0.88) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$4(0.30) & H$-$2$\rightarrow$L$+$4(-0.28) \\ 

\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.52) & H$\rightarrow$L$+$1(0.70)\\ 
\hspace{0.0mm} & H$\rightarrow$L$+$4(0.36) & H$\rightarrow$L$+$4(0.46)\\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$1(0.37)\\ 

\hspace{0.0mm} $3^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$4(-0.50) & H$\rightarrow$L$+$1(0.61) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(+0.43) & H$-$1$\rightarrow$L$+$1(-0.50) \\ 
\hspace{0.0mm} & & H$\rightarrow$L(-0.47) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/naphthalene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:naphthalene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for naphthalene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.49) & H$-$1$\rightarrow$L(-0.66) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(-0.49) & H$\rightarrow$L$+$1(-0.65) \\ 
\hspace{0.0mm} $1^1B_{2u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.62) & H$\rightarrow$L(-0.92) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(-0.30) & H$-$1$\rightarrow$L$+$1(0.27) \\ 
\hspace{0.0mm} $2^1A_{g}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$2(-0.57) & H$-$1$\rightarrow$L$+$2(-0.66) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(-0.35) & H$-$2$\rightarrow$L$+$1(-0.59) \\  
\hspace{0.0mm} $1^1B_{1g}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(-0.62) & H$\rightarrow$L$+$2(0.87) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(-0.29) & H$-$2$\rightarrow$L(-0.34) \\ 
\hspace{0.0mm} $2^1B_{3u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.49) & H$\rightarrow$L$+$1(-0.67) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.48) & H$-$1$\rightarrow$L(0.66) \\ 
\hspace{0.0mm} $2^1B_{1g}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(-0.58) & H$-$2$\rightarrow$L(-0.88) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(0.38) & H$\rightarrow$L$+2$(-0.34) \\ 
\hspace{0.0mm} $2^1B_{2u}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.60) & H$\rightarrow$L$+$1(0.90) \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.31) & H$\rightarrow$L(0.23) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/norbornadiene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:norbornadiene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for norbornadiene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.68) & H$\rightarrow$L(0.95) \\ 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.67) & H$-$1$\rightarrow$L(0.89) \\ 
\hspace{0.0mm} & & H$\rightarrow$L(-0.29) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/octatetraene_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:octatetraene_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for octatetraene.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{g}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(0.45) & H$-$1$\rightarrow$L(-0.62) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.35) & H$\rightarrow$L$+$2(-0.53) \\
\hspace{0.0mm} $1^1B_{u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.68) & H$\rightarrow$L(-0.95) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/propanamide_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:propanamide_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for propanamide.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$2(-0.54) & H$-$1$\rightarrow$L$+$2(-0.80) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$5(0.28) & H$-$1$\rightarrow$L$+$5(-0.39) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$7(-0.23) \\ 
\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$2(-0.58) & H$\rightarrow$L$+$2(-0.63) \\ 
\hspace{0.0mm} & H$\rightarrow$L-5(0.26) & H$-$1$\rightarrow$L(0.56) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$1(0.26) \\ 
\hspace{0.0mm} & & H$\rightarrow$L(-0.22) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/pyrazine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrazine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for pyrazine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.68) & H$-$1$\rightarrow$L(-0.94) \\ 
\hspace{0.0mm} $1^1A_{u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.68) & H$\rightarrow$L(-0.84) \\ 
\hspace{0.0mm} & & H$-$2$\rightarrow$L$+$1(0.39) \\ 
\hspace{0.0mm} $1^1B_{2u}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(-0.69) & H$-$1$\rightarrow$L$+$1(0.95) \\ 
\hspace{0.0mm} $1^1B_{2g}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(-0.65) & H$-$3$\rightarrow$L(0.92) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$7(0.20) & \\ 
\hspace{0.0mm} $1^1B_{1g}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$1(-0.69) & H$-$3$\rightarrow$L$+$1(0.94) \\ 
\hspace{0.0mm} $1^1B_{1u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.56) & H$\rightarrow$L$+$1(-0.85) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(-0.40) & H$-$2$\rightarrow$L(-0.45) \\ 
\hspace{0.0mm} $2^1B_{1u}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(0.61) & H$-$2$\rightarrow$L$+$1(0.84) \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.30) & H$\rightarrow$L(0.39) \\ 
\hspace{0.0mm} $2^1B_{2u}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.54) & H$-$2$\rightarrow$L(0.81) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.40) & H$\rightarrow$L$+$1(-0.41) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/pyridazine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridazine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for pyridazine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.67) & H$-$2$\rightarrow$L(-0.94) \\ 
\hspace{0.0mm} $1^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(0.64) & H$-$2$\rightarrow$L$+$1(0.94) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.65) & H$\rightarrow$L(-0.75) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.26) & H$-$1$\rightarrow$L$+$1(0.54) \\ 
\hspace{0.0mm} $2^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(0.59) & H$-$3$\rightarrow$L(0.91) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(0.26) & \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/pyridine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for pyridine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.67) & H$\rightarrow$L(0.77) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$1(0.52) \\
\hspace{0.0mm} $1^1B_{1}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(-0.62) & H$-$2$\rightarrow$L(-0.92) \\ 
\hspace{0.0mm} $2^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(0.65) & H$-$2$\rightarrow$L$+$1(0.94) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.53) & H$\rightarrow$L$+$1(0.76) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.44) & H$-$1$\rightarrow$L(-0.59) \\ 
\hspace{0.0mm} $3^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(-0.48) & H$-$1$\rightarrow$L(-0.73) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.47) & H$\rightarrow$L$+$1(-0.56) \\ 
\hspace{0.0mm} $2^1B_{2}$ & & \\ % need to figure out which state this is supposed to be
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.56) & H$-$1$\rightarrow$L$+$1(+0.77) \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.39) & H$\rightarrow$L(-0.51) \\
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/pyrimidine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrimidine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for pyrimidine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.67) & H$-$1$\rightarrow$L(-0.94) \\ 
\hspace{0.0mm} $1^1A_{2}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.66) & H$-$1$\rightarrow$L$+$1(0.94) \\ 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.66) & H$\rightarrow$L(0.77) \\ 
\hspace{0.0mm} & & H$-$2$\rightarrow$L$+$1(0.53) \\ 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(-0.51) & H$\rightarrow$L$+$1(0.81) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(-0.38) & H$-$2$\rightarrow$L(-0.49) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/pyrrole_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrrole_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for pyrrole.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(-0.55) & H$-$1$\rightarrow$L$+$1(0.71) \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$6(-0.42) & H$\rightarrow$L$+$6(-0.57) \\ 
\hspace{0.0mm} $1^1B_{2}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.67) & H$\rightarrow$L$+$1(-0.92) \\ 
\hspace{0.0mm} & & H$-$1$\rightarrow$L$+$6(-0.22) \\ 
\hspace{0.0mm} $3^1A_{1}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$6(-0.51) & H$\rightarrow$L$+$6(0.71) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L$+$1(0.45) & H$-$1$\rightarrow$L$+$1(0.57) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/tetrazine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:tetrazine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for tetrazine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.68) & H$\rightarrow$L(0.95) \\ 
\hspace{0.0mm} $1^1A_{u}$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(0.67) & H$\rightarrow$L$+$1(-0.94) \\ 
\hspace{0.0mm} $1^1B_{1g}$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(-0.67) & H$-$1$\rightarrow$L(0.82) \\ 
\hspace{0.0mm} & & H$-$2$\rightarrow$L$+$1(0.43) \\ 
\hspace{0.0mm} $1^1B_{2u}$ & & \\ 
\hspace{0.0mm} & H$-$4$\rightarrow$L(-0.61) & H$-$4$\rightarrow$L(-0.93) \\ 
\hspace{0.0mm} & H$\rightarrow$L+6(0.26) & \\ 
\hspace{0.0mm} $2^1A_{u}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(0.61) & H$-$3$\rightarrow$L(0.93) \\ 
\hspace{0.0mm} & H$\rightarrow$L+1(-0.30) & \\
\hspace{0.0mm} $1^1B_{2g}$ & & \\ 
\hspace{0.0mm} & H$-$5$\rightarrow$L(0.65) & H$-$5$\rightarrow$L(-0.92) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/thymine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:thymine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for thymine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.54) & H$-$2$\rightarrow$L(0.81) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$4(-0.22) & H$-$2$\rightarrow$L$+$4(0.30) \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(0.22) & H$-$3$\rightarrow$L(0.26) \\ 
\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(0.67) & H$\rightarrow$L(-0.90) \\ 
\hspace{0.0mm} $3^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.71) & H$-$1$\rightarrow$L(-0.88) \\ 
\hspace{0.0mm} $2^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$4(-0.52) & H$-$3$\rightarrow$L$+$4(0.64) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$4(0.29) & H$-$2$\rightarrow$L$+$4(-0.54) \\ 
\hspace{0.0mm} & & H$-$3$\rightarrow$L(-0.26) \\ 
\hspace{0.0mm} $4^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$4(0.68) & H$\rightarrow$L$+$4(0.89) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/triazine_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:triazine_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for triazine.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{1}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$1(-0.51) & H$-$2$\rightarrow$L(-0.67) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.44) & H$-$3$\rightarrow$L$+$1(0.67) \\ 
\hspace{0.0mm} $1^1A_{2}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(0.48) & H$-$3$\rightarrow$L(-0.66) \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(-0.48) & H$-$2$\rightarrow$L$+$1(-0.66) \\ 
\hspace{0.0mm} $1^1E_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$1(-0.49) & H$-$2$\rightarrow$L$+$1(-0.66) \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(-0.46) & H$-$3$\rightarrow$L(0.66) \\ 
\hspace{0.0mm} $1^1A_{2}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$1(-0.48) & H$-$1$\rightarrow$L(-0.66) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.46) & H$\rightarrow$L$+$1(-0.66) \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> CI_amps/uracil_CI_amps_table.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:uracil_CI_amps}
Singles amplitudes with magnitudes above 0.2 from the ESMF and EOM-CCSD wave functions for the calculated states for uracil.}
\begin{tabular}{l l l}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} ESMF & 
\hspace{2mm} EOM 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L(0.53) & H$-$2$\rightarrow$L(0.80) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$3(0.24) & H$-$2$\rightarrow$L$+$3(0.33) \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(0.21) & H$-$3$\rightarrow$L(0.24) \\ 
\hspace{0.0mm} $2^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L(-0.67) & H$\rightarrow$L(-0.90) \\ 
\hspace{0.0mm} $3^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L(0.50) & H$-$3$\rightarrow$L(0.76) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$3(-0.39) & H$-$2$\rightarrow$L$+$3(-0.52) \\ 
\hspace{0.0mm} $2^1A_{}^{\prime\prime}$ & & \\ 
\hspace{0.0mm} & H$-$3$\rightarrow$L$+$3(-0.51) & H$-$3$\rightarrow$L$+$3(0.62) \\ 
\hspace{0.0mm} & H$-$2$\rightarrow$L$+$3(0.27) & H$-$2$\rightarrow$L$+$3(-0.54) \\
\hspace{0.0mm} & & H$-$3$\rightarrow$L(-0.31) \\
\hspace{0.0mm} & & H$-$2$\rightarrow$L(0.23) \\
\hspace{0.0mm} & & H$-$3$\rightarrow$L$+$11(-0.21) \\
\hspace{0.0mm} $4^1A_{}^\prime$ & & \\ 
\hspace{0.0mm} & H$\rightarrow$L$+$3(0.49) & H$\rightarrow$L$+$3(0.90) \\ 
\hspace{0.0mm} & H$-$1$\rightarrow$L(0.38) & \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/acetamide_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetamide_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for acetamide.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm  & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm  
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.14 & 0.18 & 0.27 & 0.14 \\ 
\hspace{0.0mm} $2^1A'$ & 0.39 & 0.27 & 0.03 & 0.20 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/acetone_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetone_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for acetone.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 0.01 & 0.18 & 0.12 & 0.14 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.12 & 0.19 & 0.06 & 0.15 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.32 & 0.25 & 0.12 & 0.16 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/adenine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:adenine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for adenine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A'$ & 0.84 & 0.41 & 0.11 & 0.26 \\ 
\hspace{0.0mm} $3^1A'$ & 0.35 & 0.32 & 0.12 & 0.22 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.25 & 0.32 & 0.32 & 0.23 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.63 & 0.34 & 0.09 & 0.24 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/benzene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for benzene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2u}$ & 1.05 & 0.42 & 0.10 & 0.26 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.47 & 0.27 & 0.30 & 0.18 \\ 
\hspace{0.0mm} $1^1E_{1u}$ & 0.65 & 0.31 & 0.02 & 0.21 \\ 
\hspace{0.0mm} $2^1E_{2g}$ & 0.81 & 0.60 & 0.96 & 0.26 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/benzoquinone_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzoquinone_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for benzoquinone.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm  
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{u}$ & 1.03 & 0.40 & 0.19 & 0.24 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 1.09 & 0.40 & 0.26 & 0.24 \\ 
\hspace{0.0mm} $1^1B_{3g}$ & 0.58 & 0.32 & 0.13 & 0.21 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.59 & 0.34 & 0.02 & 0.23 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & 0.72 & 0.40 & 0.54 & 0.26 \\ 
\hspace{0.0mm} $2^1B_{3g}$ & 0.95 & 0.40 & 0.03 & 0.26 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/butadiene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:butadiene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for butadiene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm  
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 0.16 & 0.23 & 0.00 & 0.18 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 2.24 & 0.77 & 0.43 & 0.31 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/cyclopentadiene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopentadiene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for cyclopentadiene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 0.32 & 0.23 & 0.19 & 0.17 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 1.48 & 0.59 & 0.29 & 0.28 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/cyclopropene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopropene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for cyclopropene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 0.20 & 0.20 & 0.15 & 0.15 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.31 & 0.20 & 0.21 & 0.15 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/cytosine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cytosine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for cytosine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.40 & 0.32 & 0.19 & 0.23 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.57 & 0.21 & 0.54 & 0.16 \\ 
\hspace{0.0mm} $3^1A'$ & 0.84 & 0.37 & 0.06 & 0.23 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/ethene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:ethene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for ethene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1u}$ & 0.25 & 0.16 & 0.24 & 0.13 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/formaldehyde_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formaldehyde_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for formaldehyde.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 0.08 & 0.17 & 0.07 & 0.13 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.02 & 0.17 & 0.12 & 0.14 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.48 & 0.25 & 0.60 & 0.15 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/formamide_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formamide_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for formamide.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.01 & 0.17 & 0.16 & 0.14 \\ 
\hspace{0.0mm} $2^1A'$ & 0.02 & 0.20 & 0.08 & 0.14 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/furan_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:furan_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for furan.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 0.14 & 0.24 & 0.00 & 0.17 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 1.53 & 0.51 & 0.07 & 0.28 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 0.26 & 0.28 & 0.25 & 0.19 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/hexatriene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:hexatriene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudescalculated from the norm of the first order ESMP wave function for hexatriene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 0.18 & 0.26 & 0.04 & 0.18 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 2.72 & 1.00 & 0.72 & 0.32 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/imidazole_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:imidazole_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for imidazole.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.01 & 0.19 & 0.09 & 0.15 \\ 
\hspace{0.0mm} $2^1A'$ & 0.54 & 0.43 & 0.30 & 0.22 \\ 
\hspace{0.0mm} $3^1A'$ & 0.36 & 0.27 & 0.43 & 0.19 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/naphthalene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:naphthalene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for naphthalene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 1.02 & 0.42 & 0.11 & 0.26 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.44 & 0.33 & 0.04 & 0.21 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 0.84 & 0.42 & 0.21 & 0.26 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 0.04 & 0.31 & 0.37 & 0.20 \\ 
\hspace{0.0mm} $2^1B_{3u}$ & 0.74 & 0.33 & 0.08 & 0.22 \\ 
\hspace{0.0mm} $2^1B_{1g}$ & 1.52 & 0.49 & 0.18 & 0.27 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 0.91 & 0.36 & 0.11 & 0.23 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/norbornadiene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:norbornadiene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for norbornadiene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 0.25 & 0.25 & 0.03 & 0.18 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.32 & 0.28 & 0.20 & 0.20 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/octatetraene_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:octatetraene_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for octatetraene.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{g}$ & 3.28 & 1.15 & 0.52 & 0.33 \\ 
\hspace{0.0mm} $1^1B_{u}$ & 0.50 & 0.28 & 0.23 & 0.19 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/propanamide_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:propanamide_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for propanamide.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm  
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.03 & 0.18 & 0.16 & 0.14 \\ 
\hspace{0.0mm} $2^1A'$ & 0.37 & 0.28 & 0.06 & 0.20 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/pyrazine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrazine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for pyrazine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 0.61 & 0.34 & 0.05 & 0.23 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 0.97 & 0.36 & 0.00 & 0.25 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.39 & 0.34 & 0.22 & 0.23 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 0.64 & 0.37 & 0.09 & 0.23 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 1.18 & 0.41 & 0.09 & 0.26 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.10 & 0.28 & 0.08 & 0.19 \\ 
\hspace{0.0mm} $2^1B_{1u}$ & 0.81 & 0.32 & 0.10 & 0.22 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 0.61 & 0.35 & 0.16 & 0.23 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/pyridazine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridazine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for pyridazine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 0.52 & 0.30 & 0.11 & 0.22 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.66 & 0.31 & 0.07 & 0.22 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.90 & 0.40 & 0.02 & 0.26 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 0.95 & 0.35 & 0.24 & 0.24 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/pyridine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for pyridine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 0.33 & 0.36 & 0.34 & 0.23 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.34 & 0.24 & 0.39 & 0.17 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 0.14 & 0.26 & 0.39 & 0.19 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.04 & 0.29 & 0.19 & 0.19 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 0.63 & 0.33 & 0.11 & 0.22 \\ 
\hspace{0.0mm} $2^1B_{2}$ & 0.73 & 0.34 & 0.02 & 0.22 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/pyrimidine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrimidine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for pyrimidine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 0.90 & 0.32 & 0.31 & 0.23 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.73 & 0.33 & 0.08 & 0.23 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.48 & 0.34 & 0.11 & 0.23 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.59 & 0.38 & 0.30 & 0.23 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/pyrrole_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrrole_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for pyrrole.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & 1.07 & 0.45 & 0.04 & 0.26 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.32 & 0.25 & 0.12 & 0.18 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 0.41 & 0.29 & 0.13 & 0.19 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/tetrazine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:tetrazine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for tetrazine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 0.88 & 0.36 & 0.12 & 0.25 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 1.00 & 0.37 & 0.07 & 0.25 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 0.67 & 0.41 & 0.21 & 0.24 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.93 & 0.40 & 0.05 & 0.26 \\ 
\hspace{0.0mm} $2^1A_{u}$ & 1.86 & 0.41 & 0.72 & 0.27 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 0.93 & 0.43 & 0.10 & 0.25 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/thymine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:thymine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for thymine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.09 & 0.23 & 0.08 & 0.17 \\ 
\hspace{0.0mm} $2^1A'$ & 0.36 & 0.29 & 0.09 & 0.21 \\ 
\hspace{0.0mm} $3^1A'$ & 1.71 & 0.50 & 0.33 & 0.27 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.39 & 0.19 & 0.28 & 0.15 \\ 
\hspace{0.0mm} $4^1A'$ & 1.62 & 0.48 & 0.08 & 0.29 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/triazine_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:triazine_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for triazine.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{1}^{\prime\prime}$ & 1.37 & 0.37 & 0.16 & 0.25 \\ 
\hspace{0.0mm} $1^1A_{2}^{\prime\prime}$ & 1.01 & 0.39 & 0.18 & 0.25 \\ 
\hspace{0.0mm} $1^1E^{\prime\prime}$ & 1.22 & 0.37 & 0.23 & 0.25 \\ 
\hspace{0.0mm} $1^1A_2^\prime$ & 1.45 & 0.44 & 0.31 & 0.28 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_amps/uracil_vs_TBE_errors_w_amps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:uracil_ESMP2_vs_TBE_amps}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) errors vs. the Thiel best estimates (TBEs) and the corresponding norm of the doubles amplitudes calculated from the norm of the first order ESMP wave function for uracil.}
\begin{tabular}{l | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} lvl=0.0 error & 
\hspace{2mm} norm & 
\hspace{2mm} lvl=0.5 error & 
\hspace{2mm} norm 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.02 & 0.23 & 0.03 & 0.17 \\ 
\hspace{0.0mm} $2^1A'$ & 0.55 & 0.32 & 0.01 & 0.21 \\ 
\hspace{0.0mm} $3^1A^{\prime\prime}$ & 0.93 & 0.42 & 0.37 & 0.27 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.39 & 0.19 & 0.29 & 0.15 \\ 
\hspace{0.0mm} $4^1A'$ & 1.56 & 0.43 & 0.30 & 0.27 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/acetamide_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetamide_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for acetamide.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.80 & 4.67 & 1.13 & 5.66 & 0.14 & 5.53 & 0.27 \\ 
\hspace{0.0mm} $2^1A'$ & 7.27 & 7.85 & 0.58 & 6.88 & 0.39 & 7.30 & 0.03 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/acetone_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetone_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for acetone.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 4.40 & 3.47 & 0.93 & 4.39 & 0.01 & 4.28 & 0.12 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 9.10 & 8.48 & 0.62 & 9.22 & 0.12 & 9.16 & 0.06 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 9.40 & 8.82 & 0.58 & 9.08 & 0.32 & 9.28 & 0.12 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/adenine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:adenine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for adenine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A'$ & 5.25 & 6.52 & 1.27 & 4.41 & 0.84 & 5.36 & 0.11 \\ 
\hspace{0.0mm} $3^1A'$ & 5.25 & 5.94 & 0.69 & 4.90 & 0.35 & 5.37 & 0.12 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.12 & 6.33 & 1.21 & 4.87 & 0.25 & 5.44 & 0.32 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 5.75 & 7.00 & 1.25 & 5.12 & 0.63 & 5.84 & 0.09 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/benzene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for benzene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2u}$ & 5.08 & 6.08 & 1.00 & 4.03 & 1.05 & 4.98 & 0.10 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 6.54 & 6.22 & 0.32 & 6.07 & 0.47 & 6.24 & 0.30 \\ 
\hspace{0.0mm} $1^1E_{1u}$ & 7.13 & 7.89 & 0.76 & 6.48 & 0.65 & 7.11 & 0.02 \\ 
\hspace{0.0mm} $2^1E_{2g}$ & 8.41 & 10.65 & 2.24 & 7.60 & 0.81 & 9.37 & 0.96 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/benzoquinone_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzoquinone_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for benzoquinone.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{u}$ & 2.80 & 3.52 & 0.72 & 1.77 & 1.03 & 2.61 & 0.19 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 2.78 & 3.50 & 0.72 & 1.69 & 1.09 & 2.52 & 0.26 \\ 
\hspace{0.0mm} $1^1B_{3g}$ & 4.25 & 4.56 & 0.31 & 3.67 & 0.58 & 4.12 & 0.13 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 5.29 & 6.03 & 0.74 & 4.70 & 0.59 & 5.31 & 0.02 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & 5.60 & 8.14 & 2.54 & 4.88 & 0.72 & 6.14 & 0.54 \\ 
\hspace{0.0mm} $2^1B_{3g}$ & 6.98 & 8.27 & 1.29 & 6.03 & 0.95 & 7.01 & 0.03 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/butadiene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:butadiene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for butadiene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 6.18 & 6.29 & 0.12 & 6.02 & 0.16 & 6.18 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 6.55 & 8.85 & 2.30 & 4.31 & 2.24 & 6.98 & 0.43 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/cyclopentadiene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopentadiene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for cyclopentadiene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 5.55 & 5.40 & 0.15 & 5.23 & 0.32 & 5.36 & 0.19 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 6.31 & 8.27 & 1.96 & 4.83 & 1.48 & 6.60 & 0.29 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/cyclopropene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopropene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for cyclopropene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 6.76 & 6.44 & 0.32 & 6.56 & 0.20 & 6.61 & 0.15 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 7.06 & 6.76 & 0.30 & 6.75 & 0.31 & 6.85 & 0.21 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/cytosine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cytosine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for cytosine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 4.87 & 6.03 & 1.16 & 4.47 & 0.40 & 5.06 & 0.19 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 5.26 & 5.12 & 0.14 & 5.83 & 0.57 & 5.80 & 0.54 \\ 
\hspace{0.0mm} $3^1A'$ & 5.62 & 6.64 & 1.02 & 4.78 & 0.84 & 5.56 & 0.06 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/ethene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:ethene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for ethene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1u}$ & 7.80 & 7.77 & 0.03 & 8.05 & 0.25 & 8.04 & 0.24 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/formaldehyde_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formaldehyde_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for formaldehyde.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 3.88 & 2.93 & 0.95 & 3.96 & 0.08 & 3.81 & 0.07 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 9.10 & 8.12 & 0.98 & 9.12 & 0.02 & 8.98 & 0.12 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 9.30 & 9.22 & 0.08 & 9.78 & 0.48 & 9.90 & 0.60 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/formamide_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formamide_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for formamide.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.63 & 4.56 & 1.07 & 5.62 & 0.01 & 5.47 & 0.16 \\ 
\hspace{0.0mm} $2^1A'$ & 7.44 & 7.03 & 0.41 & 7.42 & 0.02 & 7.52 & 0.08 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/furan_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:furan_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for furan.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 6.32 & 6.34 & 0.02 & 6.18 & 0.14 & 6.32 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 6.57 & 8.04 & 1.47 & 5.04 & 1.53 & 6.50 & 0.07 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 8.13 & 8.96 & 0.83 & 7.87 & 0.26 & 8.38 & 0.25 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/hexatriene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:hexatriene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for hexatriene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 5.10 & 5.34 & 0.25 & 4.92 & 0.18 & 5.14 & 0.04 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 5.09 & 7.87 & 2.78 & 2.37 & 2.72 & 5.81 & 0.72 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/imidazole_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:imidazole_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for imidazole.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 6.81 & 6.11 & 0.70 & 6.80 & 0.01 & 6.72 & 0.09 \\ 
\hspace{0.0mm} $2^1A'$ & 6.19 & 7.08 & 0.89 & 5.65 & 0.54 & 6.49 & 0.30 \\ 
\hspace{0.0mm} $3^1A'$ & 6.93 & 7.77 & 0.84 & 7.01 & 0.08 & 7.36 & 0.43 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/naphthalene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:naphthalene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for naphthalene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 4.24 & 5.17 & 0.93 & 3.22 & 1.02 & 4.13 & 0.11 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 4.77 & 5.04 & 0.27 & 4.33 & 0.44 & 4.73 & 0.04 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 5.90 & 7.28 & 1.38 & 5.06 & 0.84 & 6.11 & 0.21 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 6.00 & 6.69 & 0.69 & 5.96 & 0.04 & 6.37 & 0.37 \\ 
\hspace{0.0mm} $2^1B_{3u}$ & 6.07 & 6.85 & 0.78 & 5.33 & 0.74 & 5.99 & 0.08 \\ 
\hspace{0.0mm} $2^1B_{1g}$ & 6.48 & 7.76 & 1.28 & 4.96 & 1.52 & 6.30 & 0.18 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 6.33 & 7.11 & 0.78 & 5.42 & 0.91 & 6.22 & 0.11 \\  
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/norbornadiene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:norbornadiene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for norbornadiene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 5.34 & 5.49 & 0.15 & 5.09 & 0.25 & 5.31 & 0.03 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 6.11 & 7.12 & 1.01 & 5.79 & 0.32 & 6.31 & 0.20 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/octatetraene_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:octatetraene_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for octatetraene.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{g}$ & 4.47 & 7.01 & 2.54 & 1.19 & 3.28 & 4.99 & 0.52 \\ 
\hspace{0.0mm} $1^1B_{u}$ & 4.66 & 4.71 & 0.05 & 4.16 & 0.50 & 4.43 & 0.23 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/propanamide_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:propanamide_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for propanamide.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.72 & 4.71 & 1.01 & 5.69 & 0.03 & 5.56 & 0.16 \\ 
\hspace{0.0mm} $2^1A'$ & 7.20 & 7.83 & 0.63 & 6.83 & 0.37 & 7.26 & 0.06 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/pyrazine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrazine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for pyrazine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 3.95 & 4.94 & 0.99 & 3.34 & 0.61 & 4.00 & 0.05 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 4.81 & 6.61 & 1.80 & 3.84 & 0.97 & 4.81 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 4.64 & 5.57 & 0.93 & 4.25 & 0.39 & 4.86 & 0.22 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 5.56 & 6.38 & 0.82 & 4.92 & 0.64 & 5.65 & 0.09 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 6.60 & 8.71 & 2.11 & 5.42 & 1.18 & 6.69 & 0.09 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 6.58 & 6.63 & 0.05 & 6.48 & 0.10 & 6.66 & 0.08 \\ 
\hspace{0.0mm} $2^1B_{1u}$ & 7.72 & 8.54 & 0.82 & 6.91 & 0.81 & 7.62 & 0.10 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 7.60 & 8.64 & 1.04 & 6.99 & 0.61 & 7.76 & 0.16 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/pyridazine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridazine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for pyridazine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 3.78 & 4.33 & 0.55 & 3.26 & 0.52 & 3.67 & 0.11 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 4.32 & 5.18 & 0.86 & 3.66 & 0.66 & 4.25 & 0.07 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 5.18 & 6.20 & 1.02 & 4.28 & 0.90 & 5.16 & 0.02 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 5.77 & 6.54 & 0.77 & 4.82 & 0.95 & 5.53 & 0.24 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/pyridine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for pyridine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 4.85 & 5.97 & 1.12 & 4.52 & 0.33 & 5.19 & 0.34 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 4.59 & 4.70 & 0.11 & 4.93 & 0.34 & 4.98 & 0.39 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 5.11 & 5.65 & 0.54 & 5.25 & 0.14 & 5.50 & 0.39 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 6.26 & 6.47 & 0.21 & 6.22 & 0.04 & 6.45 & 0.19 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 7.18 & 8.21 & 1.03 & 6.55 & 0.63 & 7.29 & 0.11 \\ 
\hspace{0.0mm} $2^1B_{2}$ & 7.27 & 8.14 & 0.87 & 6.54 & 0.73 & 7.25 & 0.02 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/pyrimidine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrimidine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for pyrimidine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 4.55 & 5.17 & 0.62 & 3.65 & 0.90 & 4.24 & 0.31 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 4.91 & 5.89 & 0.98 & 4.18 & 0.73 & 4.83 & 0.08 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 5.44 & 6.20 & 0.76 & 4.96 & 0.48 & 5.55 & 0.11 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 6.95 & 8.31 & 1.36 & 6.36 & 0.59 & 7.25 & 0.30 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/pyrrole_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrrole_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for pyrrole.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & 6.37 & 7.54 & 1.17 & 5.30 & 1.07 & 6.41 & 0.04 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 6.57 & 6.57 & 0.00 & 6.25 & 0.32 & 6.45 & 0.12 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 7.91 & 8.69 & 0.78 & 7.50 & 0.41 & 8.04 & 0.13 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/tetrazine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:tetrazine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for tetrazine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 2.24 & 3.34 & 1.10 & 1.36 & 0.88 & 2.12 & 0.12 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 3.48 & 5.39 & 1.91 & 2.48 & 1.00 & 3.55 & 0.07 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 4.73 & 5.99 & 1.26 & 4.06 & 0.67 & 4.94 & 0.21 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 4.91 & 5.96 & 1.05 & 3.98 & 0.93 & 4.86 & 0.05 \\ 
\hspace{0.0mm} $2^1A_{u}$ & 5.47 & 6.53 & 1.06 & 3.61 & 1.86 & 4.75 & 0.72 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 5.18 & 6.41 & 1.23 & 4.25 & 0.93 & 5.28 & 0.10 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/thymine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:thymine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for thymine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 4.82 & 4.26 & 0.56 & 4.91 & 0.09 & 4.90 & 0.08 \\ 
\hspace{0.0mm} $2^1A'$ & 5.20 & 5.96 & 0.76 & 4.84 & 0.36 & 5.29 & 0.09 \\ 
\hspace{0.0mm} $3^1A'$ & 6.27 & 7.50 & 1.23 & 4.56 & 1.71 & 5.94 & 0.33 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 6.16 & 5.62 & 0.54 & 6.55 & 0.39 & 6.44 & 0.28 \\ 
\hspace{0.0mm} $4^1A'$ & 6.53 & 8.68 & 2.15 & 4.91 & 1.62 & 6.45 & 0.08 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/triazine_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:triazine_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for triazine.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{1}^{\prime\prime}$ & 4.60 & 6.04 & 1.44 & 3.23 & 1.37 & 4.44 & 0.16 \\ 
\hspace{0.0mm} $1^1A_{2}^{\prime\prime}$ & 4.66 & 6.14 & 1.48 & 3.65 & 1.01 & 4.48 & 0.18 \\ 
\hspace{0.0mm} $1^1E^{\prime\prime}$ & 4.71 & 6.16 & 1.45 & 3.49 & 1.22 & 4.48 & 0.23 \\ 
\hspace{0.0mm} $1^1A_2^\prime$ & 5.79 & 6.95 & 1.16 & 4.34 & 1.45 & 5.48 & 0.31 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> ESMP2_vs_TBE/uracil_vs_TBE_errors.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:uracil_ESMP2_vs_TBE}
Absolute ESMF, ESMP2 and level shifted ESMP2 (level shift = 0.50 a.u.) results vs. the Thiel best estimates (TBEs) for uracil.}
\begin{tabular}{l| c | c c | c c | c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} ESMF & 
\hspace{2mm} error & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} error & 
\hspace{2mm} shift=0.50 a.u. & 
\hspace{2mm} error 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 4.80 & 4.24 & 0.56 & 4.82 & 0.02 & 4.83 & 0.03 \\ 
\hspace{0.0mm} $2^1A'$ & 5.35 & 6.18 & 0.83 & 4.80 & 0.55 & 5.36 & 0.01 \\ 
\hspace{0.0mm} $3^1A^{\prime\prime}$ & 6.56 & 8.98 & 2.42 & 5.63 & 0.93 & 6.93 & 0.37 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 6.10 & 5.56 & 0.54 & 6.49 & 0.39 & 6.39 & 0.29 \\ 
\hspace{0.0mm} $4^1A'$ & 6.70 & 8.12 & 1.42 & 5.14 & 1.56 & 6.40 & 0.30 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/acetamide_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetamide_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of acetamide.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 93.51 & 4.23 & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & 85.23 & 8.08 & 0.10 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/acetone_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetone_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of acetone.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 97.90 & 0.00 & 1.18 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 100.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 96.97 & 0.23 & 0.01 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/adenine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:adenine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of adenine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A'$ & 76.38 & 9.57 & 0.00 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 78.60 & 6.53 & 0.09 \\ 
\hspace{0.0mm} $3^1A'$ & 81.27 & 6.62 & 0.00 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 77.69 & 7.84 & 0.69 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/benzene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of benzene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2u}$ & 79.74 & 17.13 & 1.25 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 94.77 & 3.46 & 0.09 \\ 
\hspace{0.0mm} $1^1E_{1u}$ & 45.42 & 46.89 & 5.00 \\ 
\hspace{0.0mm} $2^1E_{2g}$ & 88.11 & 5.47 & 3.59 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/benzoquinone_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzoquinone_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of benzoquinone.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{u}$ & 66.62 & 22.22 & 2.86 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 66.83 & 21.61 & 2.52 \\ 
\hspace{0.0mm} $1^1B_{3g}$ & 71.31 & 20.76 & 1.16 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 76.71 & 15.96 & 1.60 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & 27.93 & 53.72 & 5.59 \\ 
\hspace{0.0mm} $2^1B_{3g}$ & 68.82 & 18.78 & 2.90 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/butadiene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:butadiene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of butadiene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 94.78 & 0.27 & 1.45 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 54.77 & 41.30 & 1.52 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/cyclopentadiene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopentadiene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of cyclopentadiene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & 42.65 & 56.41 & 0.13 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 99.19 & 0.59 & 0.05 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/cyclopropene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopropene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of cyclopropene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 100.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 100.00 & 0.00 & 0.00 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/cytosine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cytosine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of cytosine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A'$ & 79.24 & 9.35 & 0.54 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 81.26 & 9.49 & 0.60 \\ 
\hspace{0.0mm} $3^1A'$ & 74.66 & 15.52 & 0.69 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 80.49 & 9.57 & 0.64 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/ethene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:ethene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of ethene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1u}$ & 100.00 & 0.00 & 0.00 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/formaldehyde_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formaldehyde_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of formaldehyde.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & 92.50 & 2.04 & 0.26 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 97.80 & 0.27 & 1.12 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 100.00 & 0.00 & 0.00 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/formamide_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formamide_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of formamide.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 99.34 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & 91.20 & 0.00 & 0.00 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/furan_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:furan_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of furan.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 91.75 & 7.15 & 0.37 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 71.71 & 25.43 & 1.15 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 64.33 & 30.51 & 2.62 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/hexatriene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:hexatriene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of hexatriene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{g}$ & 43.16 & 51.05 & 1.31 \\ 
\hspace{0.0mm} $1^1B_{u}$ & 46.50 & 26.71 & 20.85 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/imidazole_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:imidazole_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of imidazole.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 84.99 & 8.79 & 1.90 \\ 
\hspace{0.0mm} $2^1A'$ & 75.30 & 20.32 & 0.86 \\ 
\hspace{0.0mm} $3^1A'$ & 88.29 & 6.96 & 0.30 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/naphthalene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:naphthalene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of naphthalene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 71.64 & 12.61 & 1.91 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 84.65 & 7.18 & 0.92 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 57.47 & 19.95 & 1.18 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 54.81 & 25.21 & 0.02 \\ 
\hspace{0.0mm} $2^1B_{3u}$ & 37.34 & 39.74 & 2.00 \\ 
\hspace{0.0mm} $2^1B_{1g}$ & 81.32 & 4.94 & 1.69 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 80.81 & 7.34 & 1.77 \\ 
\hspace{0.0mm} $3^1A_{g}$ & 49.10 & 28.97 & 0.15 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/norbornadiene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:norbornadiene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of norbornadiene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 99.93 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 99.47 & 0.00 & 0.53 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/octatetraene_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:octatetraene_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of octatetraene.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{g}$ & 38.21 & 46.53 & 0.67 \\ 
\hspace{0.0mm} $1^1B_{u}$ & 36.52 & 46.90 & 0.00 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/propanamide_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:propanamide_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of propanamide.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 97.83 & 0.52 & 0.66 \\ 
\hspace{0.0mm} $2^1A'$ & 85.53 & 12.06 & 0.60 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/pyrazine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrazine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of pyrazine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 81.32 & 10.79 & 1.98 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 78.63 & 17.69 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 78.34 & 14.48 & 2.14 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 71.18 & 20.54 & 1.83 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 71.21 & 20.48 & 1.69 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 92.51 & 4.53 & 0.00 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 86.97 & 7.43 & 3.21 \\ 
\hspace{0.0mm} $2^1B_{1u}$ & 90.31 & 3.76 & 3.15 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/pyridazine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridazine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of pyridazine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 87.74 & 8.18 & 1.80 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 86.20 & 8.37 & 2.77 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 79.39 & 17.82 & 0.26 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 74.52 & 21.37 & 1.33 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/pyridine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of pyridine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 78.62 & 17.20 & 1.25 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 88.99 & 3.14 & 2.28 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 88.52 & 3.97 & 1.96 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 74.85 & 19.76 & 0.82 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 62.70 & 30.38 & 1.14 \\ 
\hspace{0.0mm} $2^1B_{2}$ & 45.87 & 45.28 & 4.91 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/pyrimidine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrimidine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of pyrimidine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 84.42 & 6.35 & 1.80 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 83.35 & 8.23 & 1.23 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 75.86 & 19.81 & 2.27 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 67.47 & 24.97 & 0.74 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/pyrrole_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrrole_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of pyrrole.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & 76.61 & 21.95 & 0.94 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 88.43 & 10.67 & 0.42 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 68.47 & 27.59 & 2.63 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/tetrazine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:tetrazine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of tetrazine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 86.53 & 10.71 & 0.59 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 83.26 & 11.30 & 2.09 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 86.75 & 10.76 & 1.33 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 75.30 & 20.55 & 1.02 \\ 
\hspace{0.0mm} $2^1A_{u}$ & 79.40 & 16.40 & 1.06 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 70.51 & 24.45 & 1.02 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/thymine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:thymine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of thymine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 81.88 & 10.38 & 0.24 \\ 
\hspace{0.0mm} $2^1A'$ & 82.75 & 7.70 & 0.00 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 83.17 & 5.98 & 0.71 \\ 
\hspace{0.0mm} $3^1A'$ & 71.05 & 21.01 & 0.02 \\ 
\hspace{0.0mm} $4^1A'$ & 76.55 & 13.02 & 0.02 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/triazine_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:triazine_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of triazine.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{1}^{\prime\prime}$ & 76.65 & 13.15 & 1.41 \\ 
\hspace{0.0mm} $1^1A_{2}^{\prime\prime}$ & 79.27 & 12.32 & 1.11 \\ 
\hspace{0.0mm} $1^1E^{\prime\prime}$ & 79.27 & 13.18 & 0.69 \\ 
\hspace{0.0mm} $1^1A_2^\prime$ & 76.20 & 18.86 & 2.63 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> SA-CAS percentages/uracil_SA_CAS_percentages.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:uracil_SA_CAS_percent}
SA-CASSCF percentages for the amount of singles, doubles, and triples character for the excitations of uracil.}
\begin{tabular}{l| c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} \%singles & 
\hspace{2mm} \%doubles & 
\hspace{2mm} \%triples 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 81.94 & 9.81 & 0.14 \\ 
\hspace{0.0mm} $2^1A'$ & 83.11 & 6.81 & 0.01 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 83.11 & 6.14 & 0.58 \\ 
\hspace{0.0mm} $3^1A'$ & 72.34 & 18.53 & 0.03 \\ 
\hspace{0.0mm} $4^1A'$ & 77.40 & 12.86 & 0.01 \\ 
\hspace{0.0mm} $3^1A^{\prime\prime}$ & 61.21 & 27.02 & 1.23 \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> eV values/acetamide_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetamide_vs_all_methods}
All methods singlet excitation energies in eV for molecule acetamide.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.80 & 5.54 & 5.80 & 5.77 & 5.71 & 5.69 & 5.66 & 5.53 \\ 
 \hspace{0.0mm} $2^1A'$ & 7.27 & 7.21 & 7.27 & 7.66 & 7.85 & 7.67 & 6.88 & 7.30 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/acetone_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetone_vs_all_methods}
All methods singlet excitation energies in eV for molecule acetone.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 4.40 & 4.18 & 4.42 & 4.52 & 4.43 & 4.40 & 4.39 & 4.28 \\ 
 \hspace{0.0mm} $1^1B_{1}$ & 9.10 & 9.10 & 9.27 & 9.29 & 9.26 & 9.17 & 9.22 & 9.16 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 9.40 & 9.16 & 9.31 & 9.74 & 9.87 & 9.65 & 9.08 & 9.28 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/adenine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:adenine_vs_all_methods}
All methods singlet excitation energies in eV for molecule adenine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A'$ & 5.25 & 5.13 & 5.20 & 5.28 & 5.37 & 5.18 & 4.41 & 5.36 \\ 
 \hspace{0.0mm} $3^1A'$ & 5.25 & 5.20 & 5.30 & 5.42 & 5.61 & 5.39 & 4.90 & 5.37 \\ 
 \hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.12 & 6.15 & 5.21 & 5.27 & 5.58 & 5.34 & 4.87 & 5.44 \\ 
 \hspace{0.0mm} $2^1A^{\prime\prime}$ & 5.75 & 6.86 & 5.97 & 5.91 & 6.19 & 5.96 & 5.12 & 5.84 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/benzene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzene_vs_all_methods}
All methods singlet excitation energies in eV for molecule benzene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2u}$ & 5.08 & 4.84 & 5.05 & 5.27 & 5.19 & 5.07 & 4.03 & 4.98 \\ 
 \hspace{0.0mm} $1^1B_{1u}$ & 6.54 & 6.30 & 6.45 & 6.68 & 6.74 & 6.68 & 6.07 & 6.24 \\ 
 \hspace{0.0mm} $1^1E_{1u}$ & 7.13 & 7.03 & 7.07 & 7.44 & 7.65 & 7.45 & 6.48 & 7.11 \\ 
 \hspace{0.0mm} $2^1E_{2g}$ & 8.41 & 7.90 & 8.21 & 9.03 & 9.21 & 8.43 & 7.60 & 9.37 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/benzoquinone_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzoquinone_vs_all_methods}
All methods singlet excitation energies in eV for molecule benzoquinone.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{u}$ & 2.80 & 2.50 & 2.80 & 2.92 & 3.19 & 2.85 & 1.77 & 2.61 \\ 
 \hspace{0.0mm} $1^1B_{1g}$ & 2.78 & 2.50 & 2.78 & 2.81 & 3.07 & 2.75 & 1.69 & 2.52 \\ 
 \hspace{0.0mm} $1^1B_{3g}$ & 4.25 & 4.19 & 4.25 & 4.69 & 4.93 & 4.59 & 3.67 & 4.12 \\ 
 \hspace{0.0mm} $1^1B_{1u}$ & 5.29 & 5.15 & 5.29 & 5.59 & 5.89 & 5.62 & 4.70 & 5.31 \\ 
 \hspace{0.0mm} $1^1B_{3u}$ & 5.60 & 5.15 & 5.60 & 5.69 & 6.55 & 5.82 & 4.88 & 6.14 \\ 
 \hspace{0.0mm} $2^1B_{3g}$ & 6.98 & 6.34 & 6.98 & 7.36 & 7.62 & 7.27 & 6.03 & 7.01 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/butadiene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:butadiene_vs_all_methods}
All methods singlet excitation energies in eV for molecule butadiene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 6.18 & 6.23 & 6.47 & 6.49 & 6.72 & 6.58 & 6.02 & 6.18 \\ 
 \hspace{0.0mm} $2^1A_{g}$ & 6.55 & 6.27 & 6.83 & 7.63 & 7.42 & 6.77 & 4.31 & 6.98 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/cyclopentadiene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopentadiene_vs_all_methods}
All methods singlet excitation energies in eV for molecule cyclopentadiene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 5.55 & 5.27 & 5.51 & 5.69 & 5.87 & 5.73 & 5.23 & 5.36 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 6.31 & 6.31 & 6.31 & 7.05 & 7.05 & 6.61 & 4.83 & 6.60 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/cyclopropene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopropene_vs_all_methods}
All methods singlet excitation energies in eV for molecule cyclopropene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 6.76 & 6.36 & 6.76 & 6.96 & 6.96 & 6.90 & 6.56 & 6.61 \\ 
 \hspace{0.0mm} $1^1B_{2}$ & 7.06 & 7.45 & 7.06 & 7.17 & 7.24 & 7.10 & 6.75 & 6.85 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/cytosine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cytosine_vs_all_methods}
All methods singlet excitation energies in eV for molecule cytosine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A'$ & 4.66 & 4.39 & 4.68 & 4.80 & 4.98 & 4.72 & N/A & N/A \\
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 4.87 & 5.00 & 5.12 & 5.13 & 5.45 & 5.16 & 4.47 & 5.06 \\ 
 \hspace{0.0mm} $2^1A^{\prime\prime}$ & 5.26 & 6.53 & 5.54 & 5.01 & 5.99 & 5.52 & 5.83 & 5.80 \\ 
 \hspace{0.0mm} $3^1A'$ & 5.62 & 5.36 & 5.54 & 5.71 & 5.95 & 5.61 & 4.78 & 5.56 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/ethene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:ethene_vs_all_methods}
All methods singlet excitation energies in eV for molecule ethene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1u}$ & 7.80 & 7.98 & 8.62 & 8.40 & 8.51 & 8.37 & 8.05 & 8.04 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/formaldehyde_all_methods.tex <==
\begin{table}[htp]
\caption{
\label{tab:formaldehyde_vs_all_methods}
All methods singlet excitation energies in eV for molecule formaldehyde.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 3.88 & 3.91 & 3.98 & 4.09 & 3.97 & 3.95 & 3.96 & 3.81 \\ 
 \hspace{0.0mm} $1^1B_{1}$ & 9.10 & 9.09 & 9.14 & 9.35 & 9.26 & 9.18 & 9.12 & 8.98 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 9.30 & 9.77 & 9.31 & 10.34 & 10.54 & 10.45 & 9.78 & 9.90 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/formamide_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formamide_vs_all_methods}
All methods singlet excitation energies in eV for molecule formamide.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt]
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.63 & 5.61 & 5.63 & 5.76 & 5.66 & 5.65 & 5.62 & 5.47 \\ 
 \hspace{0.0mm} $2^1A'$ & 7.44 & 7.41 & 7.44 & 8.15 & 8.52 & 8.27 & 7.42 & 7.52 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/furan_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:furan_vs_all_methods}
All methods singlet excitation energies in eV for molecule furan.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 6.32 & 6.04 & 6.43 & 6.43 & 6.80 & 6.60 & 6.18 & 6.32 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 6.57 & 6.16 & 6.52 & 6.87 & 6.89 & 6.62 & 5.04 & 6.50 \\ 
 \hspace{0.0mm} $3^1A_{1}$ & 8.13 & 7.66 & 8.22 & 8.83 & 8.83 & 8.53 & 7.87 & 8.38 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/hexatriene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:hexatriene_vs_all_methods}
All methods singlet excitation energies in eV for molecule hexatriene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{u}$ & 5.10 & 5.01 & 5.31 & 5.41 & 5.72 & 5.58 & 4.92 & 5.14 \\ 
 \hspace{0.0mm} $2^1A_{g}$ & 5.09 & 5.20 & 5.42 & 6.67 & 6.61 & 5.72 & 2.37 & 5.81 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/imidazole_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:imidazole_vs_all_methods}
All methods singlet excitation energies in eV for molecule imidazole.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 6.81 & 6.52 & 6.81 & 6.86 & 7.01 & 6.82 & 6.80 & 6.72 \\ 
 \hspace{0.0mm} $2^1A'$ & 6.19 & 6.72 & 6.19 & 6.73 & 6.80 & 6.58 & 5.65 & 6.49 \\ 
 \hspace{0.0mm} $3^1A'$ & 6.93 & 7.15 & 6.93 & 7.28 & 7.27 & 7.10 & 7.01 & 7.36 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/naphthalene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:naphthalene_vs_all_methods}
All methods singlet excitation energies in eV for molecule naphthalene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 4.24 & 4.03 & 4.24 & 4.45 & 4.41 & 4.27 & 3.22 & 4.13 \\ 
 \hspace{0.0mm} $1^1B_{2u}$ & 4.77 & 4.56 & 4.77 & 4.96 & 5.21 & 5.03 & 4.33 & 4.73 \\ 
 \hspace{0.0mm} $2^1A_{g}$ & 5.90 & 5.39 & 5.90 & 6.22 & 6.23 & 5.98 & 5.06 & 6.11 \\ 
 \hspace{0.0mm} $1^1B_{1g}$ & 6.00 & 5.53 & 6.00 & 6.21 & 6.53 & 6.07 & 5.96 & 6.37 \\ 
 \hspace{0.0mm} $2^1B_{3u}$ & 6.07 & 5.54 & 6.07 & 6.25 & 6.55 & 6.33 & 5.33 & 5.99 \\ 
 \hspace{0.0mm} $2^1B_{1g}$ & 6.48 & 5.87 & 6.48 & 6.82 & 6.97 & 6.79 & 4.96 & 6.30 \\ 
 \hspace{0.0mm} $2^1B_{2u}$ & 6.33 & 5.93 & 6.33 & 6.57 & 6.77 & 6.57 & 5.42 & 6.22 \\ 
 \hspace{0.0mm} $3^1A_{g}$ & 6.71 & 6.04 & 6.71 & 7.34 & 7.77 & 6.90 & N/A & N/A \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/norbornadiene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:norbornadiene_vs_all_methods}
All methods singlet excitation energies in eV for molecule norbornadiene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{2}$ & 5.34 & 5.28 & 5.34 & 5.57 & 5.80 & 5.64 & 5.09 & 5.31 \\ 
 \hspace{0.0mm} $1^1B_{2}$ & 6.11 & 6.20 & 6.11 & 6.37 & 6.69 & 6.49 & 5.79 & 6.31 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/octatetraene_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:octatetraene_vs_all_methods}
All methods singlet excitation energies in eV for molecule octatetraene.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{g}$ & 4.47 & 4.38 & 4.64 & 5.87 & 5.99 & 4.97 & 1.19 & 4.99 \\ 
 \hspace{0.0mm} $1^1B_{u}$ & 4.66 & 4.42 & 4.70 & 4.72 & 5.07 & 4.94 & 4.16 & 4.43 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/propanamide_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:propanamide_vs_all_methods}
All methods singlet excitation energies in eV for molecule propanamide.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 5.72 & 5.48 & 5.72 & 5.78 & 5.74 & 5.72 & 5.69 & 5.56 \\ 
 \hspace{0.0mm} $2^1A'$ & 7.20 & 7.28 & 7.20 & 7.56 & 7.80 & 7.62 & 6.83 & 7.26 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/pyrazine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrazine_vs_all_methods}
All methods singlet excitation energies in eV for molecule pyrazine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 3.95 & 3.63 & 4.12 & 4.26 & 4.42 & 4.24 & 3.34 & 4.00 \\ 
 \hspace{0.0mm} $1^1A_{u}$ & 4.81 & 4.52 & 4.70 & 4.95 & 5.29 & 5.05 & 3.84 & 4.81 \\ 
 \hspace{0.0mm} $1^1B_{2u}$ & 4.64 & 4.75 & 4.85 & 5.13 & 5.14 & 5.02 & 4.25 & 4.86 \\ 
 \hspace{0.0mm} $1^1B_{2g}$ & 5.56 & 5.17 & 5.68 & 5.92 & 6.02 & 5.74 & 4.92 & 5.65 \\ 
 \hspace{0.0mm} $1^1B_{1g}$ & 6.60 & 6.13 & 6.41 & 6.70 & 7.13 & 6.75 & 5.42 & 6.69 \\ 
 \hspace{0.0mm} $1^1B_{1u}$ & 6.58 & 6.70 & 6.89 & 7.10 & 7.18 & 7.07 & 6.48 & 6.66 \\ 
 \hspace{0.0mm} $2^1B_{1u}$ & 7.72 & 7.57 & 7.79 & 8.13 & 8.34 & 8.06 & 6.91 & 7.62 \\ 
 \hspace{0.0mm} $2^1B_{2u}$ & 7.60 & 7.70 & 7.65 & 8.07 & 8.29 & 8.05 & 6.99 & 7.76 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/pyridazine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridazine_vs_all_methods}
All methods singlet excitation energies in eV for molecule pyridazine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt]
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 3.78 & 3.48 & 3.78 & 3.90 & 4.11 & 3.92 & 3.26 & 3.67 \\ 
 \hspace{0.0mm} $1^1A_{2}$ & 4.32 & 3.66 & 4.32 & 4.40 & 4.76 & 4.49 & 3.66 & 4.25 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 5.18 & 4.86 & 5.18 & 5.37 & 5.35 & 5.22 & 4.28 & 5.16 \\ 
 \hspace{0.0mm} $2^1A_{2}$ & 5.77 & 5.09 & 5.77 & 5.81 & 6.00 & 5.74 & 4.82 & 5.53 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/pyridine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridine_vs_all_methods}
All methods singlet excitation energies in eV for molecule pyridine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{2}$ & 4.85 & 4.84 & 5.02 & 5.32 & 5.27 & 5.15 & 4.52 & 5.19 \\ 
 \hspace{0.0mm} $1^1B_{1}$ & 4.59 & 4.91 & 5.14 & 5.12 & 5.25 & 5.05 & 4.93 & 4.98 \\ 
 \hspace{0.0mm} $2^1A_{2}$ & 5.11 & 5.17 & 5.47 & 5.39 & 5.73 & 5.50 & 5.25 & 5.50 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 6.26 & 6.42 & 6.39 & 6.88 & 6.94 & 6.85 & 6.22 & 6.45 \\ 
 \hspace{0.0mm} $3^1A_{1}$ & 7.18 & 7.23 & 7.46 & 7.72 & 7.94 & 7.70 & 6.55 & 7.29 \\ 
 \hspace{0.0mm} $2^1B_{2}$ & 7.27 & 7.48 & 7.29 & 7.61 & 7.81 & 7.59 & 6.54 & 7.25 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/pyrimidine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrimidine_vs_all_methods}
All methods singlet excitation energies in eV for molecule pyrimidine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{1}$ & 4.55 & 3.81 & 4.44 & 4.49 & 4.70 & 4.50 & 3.65 & 4.24 \\ 
 \hspace{0.0mm} $1^1A_{2}$ & 4.91 & 4.12 & 4.81 & 4.84 & 5.12 & 4.93 & 4.18 & 4.83 \\ 
 \hspace{0.0mm} $1^1B_{2}$ & 5.44 & 4.93 & 5.24 & 5.51 & 5.49 & 5.36 & 4.96 & 5.55 \\ 
 \hspace{0.0mm} $2^1A_{1}$ & 6.95 & 6.72 & 6.64 & 7.12 & 7.17 & 7.06 & 6.36 & 7.25 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/pyrrole_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrrole_vs_all_methods}
All methods singlet excitation energies in eV for molecule pyrrole.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $2^1A_{1}$ & 6.37 & 5.92 & 6.31 & 6.61 & 6.61 & 6.40 & 5.30 & 6.41 \\ 
 \hspace{0.0mm} $1^1B_{2}$ & 6.57 & 6.00 & 6.33 & 6.83 & 6.87 & 6.71 & 6.25 & 6.45 \\ 
 \hspace{0.0mm} $3^1A_{1}$ & 7.91 & 7.46 & 8.17 & 8.44 & 8.44 & 8.17 & 7.50 & 8.04 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/tetrazine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:tetrazine_vs_all_methods}
All methods singlet excitation energies in eV for molecule tetrazine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1B_{3u}$ & 2.24 & 1.96 & 2.24 & 2.47 & 2.71 & 2.53 & 1.36 & 2.12 \\ 
 \hspace{0.0mm} $1^1A_{u}$ & 3.48 & 3.06 & 3.48 & 3.67 & 4.07 & 3.79 & 2.48 & 3.55 \\ 
 \hspace{0.0mm} $1^1B_{1g}$ & 4.73 & 4.51 & 4.73 & 5.10 & 5.32 & 4.97 & 4.06 & 4.94 \\ 
 \hspace{0.0mm} $1^1B_{2u}$ & 4.91 & 4.89 & 4.91 & 5.20 & 5.27 & 5.12 & 3.98 & 4.86 \\ 
 \hspace{0.0mm} $2^1A_{u}$ & 5.47 & 5.28 & 5.47 & 5.50 & 5.70 & 5.46 & 3.61 & 4.75 \\ 
 \hspace{0.0mm} $1^1B_{2g}$ & 5.18 & 5.05 & 5.18 & 5.53 & 5.70 & 5.34 & 4.25 & 5.28 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/thymine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:thymine_vs_all_methods}
All methods singlet excitation energies in eV for molecule thymine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt]
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 4.82 & 4.39 & 4.94 & 4.94 & 5.14 & 4.98 & 4.91 & 4.90 \\ 
 \hspace{0.0mm} $2^1A'$ & 5.20 & 4.88 & 5.06 & 5.39 & 5.60 & 5.34 & 4.84 & 5.29 \\ 
 \hspace{0.0mm} $3^1A'$ & 6.27 & 5.88 & 6.15 & 6.46 & 6.78 & 6.34 & 4.56 & 5.94 \\ 
 \hspace{0.0mm} $2^1A^{\prime\prime}$ & 6.16 & 5.91 & 6.38 & 6.33 & 6.57 & 6.45 & 6.55 & 6.44 \\ 
 \hspace{0.0mm} $4^1A'$ & 6.53 & 6.10 & 6.52 & 6.80 & 7.05 & 6.71 & 4.91 & 6.45 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/triazine_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:triazine_vs_all_methods}
All methods singlet excitation energies in eV for molecule triazine.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A_{1}^{\prime\prime}$ & 4.60 & 3.90 & 4.60 & 4.70 & 4.96 & 4.78 & 3.23 & 4.44 \\ 
 \hspace{0.0mm} $1^1A_{2}^{\prime\prime}$ & 4.66 & 4.08 & 4.68 & 4.80 & 4.98 & 4.76 & 3.65 & 4.48 \\ 
 \hspace{0.0mm} $1^1E^{\prime\prime}$ & 4.71 & 4.36 & 4.71 & 4.77 & 5.01 & 4.81 & 3.49 & 4.48 \\ 
 \hspace{0.0mm} $1^1A_2^\prime$ & 5.79 & 5.33 & 5.79 & 5.82 & 5.84 & 5.71 & 4.34 & 5.48 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> eV values/uracil_all_methods.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:uracil_vs_all_methods}
All methods singlet excitation energies in eV for molecule uracil.}
\begin{tabular}{l| c c c c c c c c}
\hline\hline
\hspace{2mm} State & 
\hspace{2mm} TBE & 
\hspace{2mm} CASPT2\textsuperscript{a} & 
\hspace{2mm} CASPT2\textsuperscript{b} & 
\hspace{2mm} CC2 & 
\hspace{2mm} CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} lvl-ESMP2 
\\[2pt] 
\hline 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 4.80 & 4.54 & 4.90 & 4.91 & 5.11 & 4.90 & 4.82 & 4.83 \\ 
 \hspace{0.0mm} $2^1A'$ & 5.35 & 5.00 & 5.23 & 5.52 & 5.70 & 5.44 & 4.80 & 5.36 \\ 
 \hspace{0.0mm} $3^1A'$ & 6.26 & 5.82 & 6.15 & 6.43 & 6.76 & 6.29 & N/A & N/A \\
 \hspace{0.0mm} $3^1A^{\prime\prime}$ & 6.56 & 6.37 & 6.97 & 6.73 & 7.68 & 6.77 & 5.63 & 6.93 \\ 
 \hspace{0.0mm} $2^1A^{\prime\prime}$ & 6.10 & 6.00 & 6.27 & 6.26 & 6.50 & 6.32 & 6.49 & 6.39 \\ 
 \hspace{0.0mm} $4^1A'$ & 6.70 & 6.46 & 6.75 & 6.96 & 7.19 & 6.87 & 5.14 & 6.40 \\ 
 \hline\hline 
\end{tabular} 
\end{table} 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> main_paper_tables/TD-DFT_averages.tex <==
\begin{table*}[htbp]
\caption{Mean unsigned errors and standard deviations for TD-DFT calculations
\cite{Thiel-BM-TDDFT}
using the TZVP basis set. The states that ESMP2 found to have strong doubly excited character, the states highlighted red in Table 1, have been omitted from these averages.
\label{table:tddft_mue}
}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c c c c c c|}
\hline
\hspace{6mm} & 
\hspace{6mm} BP86 & 
\hspace{6mm} B3LYP & 
\hspace{6mm} BHLYP & 
\hspace{6mm} DFT/MRCI & 
\hspace{6mm} ESMP2 & 
\hspace{6mm} $\epsilon$-ESMP2 \\ 
\hline
\hspace{0.0mm} Aldehydes, Ketones, Amides & 0.55 $\pm$ 0.35 & 0.29 $\pm$ 0.19 & 0.35 $\pm$ 0.44 & 0.34 $\pm$ 0.21 & 0.39 $\pm$ 0.37 & 0.17 $\pm$ 0.16 \\ 
\hspace{0.0mm} Conjugated Polyenes & 0.52 $\pm$ 0.32 & 0.40 $\pm$ 0.22 & 0.22 $\pm$ 0.11 & 0.22 $\pm$ 0.13 & 0.27 $\pm$ 0.16 & 0.13 $\pm$ 0.13 \\ 
\hspace{0.0mm} Conjugated Rings & 0.51 $\pm$ 0.33 & 0.34 $\pm$ 0.19 & 0.33 $\pm$ 0.27 & 0.19 $\pm$ 0.17 & 0.60 $\pm$ 0.40 & 0.15 $\pm$ 0.10 \\ 
\hspace{0.0mm} Heterocycles & 0.44 $\pm$ 0.29 & 0.21 $\pm$ 0.18 & 0.49 $\pm$ 0.26 & 0.17 $\pm$ 0.12 & 0.68 $\pm$ 0.42 & 0.17 $\pm$ 0.14 \\ 
\hspace{0.0mm} Nucleobases & 0.82 $\pm$ 0.30 & 0.47 $\pm$ 1.14 & 0.57 $\pm$ 0.27 & 0.16 $\pm$ 0.13 & 0.68 $\pm$  0.52 & 0.19 $\pm$ 0.15 \\ \hline
\hspace{0.0mm} All & 0.55 $\pm$ 0.34 & 0.30 $\pm$ 0.53 & 0.44 $\pm$ 0.31 & 0.21 $\pm$ 0.16 & 0.60 $\pm$ 0.43 & 0.17 $\pm$ 0.14 \\ \hline
\end{tabular}}
\end{table*}


==> main_paper_tables/pi_system_size_averages.tex <==
\begin{table*}[htbp]
\caption{Mean unsigned errors in eV for different $\pi$ system sizes.
The states that ESMP2 identified as having large doubly excited character have been omitted from these values, see the red-highlighted states in Table 1.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c c c c c c c|}
\hline
\multicolumn{1}{|l|}{$\pi$ system size} & 
\hspace{2mm} CASPT2 a & 
\hspace{2mm} CASPT2 b & 
\hspace{2mm} CC2 & 
\hspace{2mm} EOM-CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} $\epsilon$-ESMP2 \\ \hline
\hspace{0.0mm} 2 & 0.19 $\pm$ 0.17 & 0.11 $\pm$ 0.24 & 0.32 $\pm$ 0.27 & 0.39 $\pm$ 0.36 & 0.28 $\pm$ 0.34 & 0.21 $\pm$ 0.14 & 0.17 $\pm$ 0.16 \\ 
\hspace{0.0mm} 3 & 0.12 $\pm$ 0.11 & 0.00 $\pm$ 0.00 & 0.28 $\pm$ 0.26 & 0.40 $\pm$ 0.43 & 0.30 $\pm$ 0.32 & 0.16 $\pm$ 0.18 & 0.13 $\pm$ 0.09 \\ 
\hspace{0.0mm} 4 & 0.17 $\pm$ 0.16 & 0.17 $\pm$ 0.18 & 0.23 $\pm$ 0.12 & 0.43 $\pm$ 0.16 & 0.29 $\pm$ 0.16 & 0.24 $\pm$ 0.12 & 0.09 $\pm$ 0.13 \\ 
\hspace{0.0mm} 5 & 0.41 $\pm$ 0.13 & 0.10 $\pm$ 0.10 & 0.38 $\pm$ 0.20 & 0.43 $\pm$ 0.18 & 0.21 $\pm$ 0.15 & 0.35 $\pm$ 0.34 & 0.17 $\pm$ 0.14 \\ 
\hspace{0.0mm} 6 & 0.31 $\pm$ 0.22 & 0.11 $\pm$ 0.13 & 0.25 $\pm$ 0.17 & 0.42 $\pm$ 0.20 & 0.24 $\pm$ 0.17 & 0.75 $\pm$ 0.39 & 0.17 $\pm$ 0.14 \\ 
\hspace{0.0mm} 8 & 0.34 $\pm$ 0.25 & 0.10 $\pm$ 0.11 & 0.22 $\pm$ 0.14 & 0.52 $\pm$ 0.30 & 0.17 $\pm$ 0.11 & 0.74 $\pm$ 0.47 & 0.20 $\pm$ 0.16 \\ 
\hspace{0.0mm} 10 & 0.49 $\pm$ 0.33 & 0.03 $\pm$ 0.07 & 0.24 $\pm$ 0.15 & 0.44 $\pm$ 0.23 & 0.17 $\pm$ 0.09 & 0.69 $\pm$ 0.41 & 0.16 $\pm$ 0.10 \\ \hline
\multicolumn{1}{|l|}{5 or less} & 0.24 $\pm$ 0.18 & 0.09 $\pm$ 0.17 & 0.32 $\pm$ 0.23 & 0.41 $\pm$ 0.31 & 0.26 $\pm$ 0.27 & 0.24 $\pm$ 0.23 & 0.16 $\pm$ 0.13 \\ 
\multicolumn{1}{|l|}{6 or more} & 0.35 $\pm$ 0.25 & 0.09 $\pm$ 0.09 & 0.24 $\pm$ 0.16 & 0.45 $\pm$ 0.24 & 0.09 $\pm$ 0.21 & 0.74 $\pm$ 0.41 & 0.18 $\pm$ 0.14 \\ \hline
\end{tabular}}
\label{pi sysstem size averages}
\end{table*}


==> main_paper_tables/wavefunction_averages.tex <==
% this has been updated with the new selection of molecules to include
% see SI document for other versions of this table
\begin{table*}[htbp]
\caption{Mean unsigned errors and standard deviations in eV
for molecular structure groups.
States with no ESMF solution
and those flagged by ESMP2 as having substantial doubly excited
character (red rows in Table 1) are excluded.
\label{tab:wfn_mue}
}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c c c c c c c|}
\hline
\hspace{2mm} & 
\hspace{2mm} CASPT2 a & 
\hspace{2mm} CASPT2 b & 
\hspace{2mm} CC2 & 
\hspace{2mm} EOM-CCSD & 
\hspace{2mm} CC3 & 
\hspace{2mm} ESMP2 & 
\hspace{2mm} $\epsilon$-ESMP2 \\ \hline
\hspace{0.0mm} Aldehydes, Ketones, Amides & 0.20 $\pm$ 0.18 & 0.02 $\pm$ 0.05 & 0.29 $\pm$ 0.26 & 0.45 $\pm$ 0.38 & 0.26 $\pm$ 0.31 & 0.39 $\pm$ 0.37 & 0.17 $\pm$ 0.16 \\ 
\hspace{0.0mm} Conjugated Polyenes & 0.14 $\pm$ 0.09 & 0.34 $\pm$ 0.34 & 0.32 $\pm$ 0.22 & 0.57 $\pm$ 0.13 & 0.43 $\pm$ 0.12 & 0.27 $\pm$ 0.16 & 0.13 $\pm$ 0.13 \\ 
\hspace{0.0mm} Conjugated Rings & 0.34 $\pm$ 0.19 & 0.01 $\pm$ 0.03 & 0.24 $\pm$ 0.12 & 0.41 $\pm$ 0.23 & 0.18 $\pm$ 0.12 & 0.60 $\pm$ 0.40 & 0.15 $\pm$ 0.10 \\ 
\hspace{0.0mm} Heterocycles & 0.34 $\pm$ 0.21 & 0.10 $\pm$ 0.13 & 0.28 $\pm$ 0.19 & 0.43 $\pm$ 0.19 & 0.23 $\pm$ 0.16 & 0.68 $\pm$ 0.42 & 0.17 $\pm$ 0.14 \\ 
\hspace{0.0mm} Nucleobases & 0.40 $\pm$ 0.35 & 0.14 $\pm$ 0.10 & 0.20 $\pm$ 0.12 & 0.46 $\pm$ 0.31 & 0.15 $\pm$ 0.09 & 0.68 $\pm$ 0.52 & 0.19 $\pm$ 0.15 \\ \hline
\hspace{0.0mm} All & 0.32 $\pm$ 0.24 & 0.09 $\pm$ 0.13 & 0.26 $\pm$ 0.18 & 0.44 $\pm$ 0.26 & 0.22 $\pm$ 0.19 & 0.60 $\pm$ 0.43 & 0.17 $\pm$ 0.14 \\ \hline
\end{tabular}}
\end{table*}


==> overlaps-needs to be double checked/acetamide_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetamide_overlaps}
Overlap between ground and other calculated excited states for acetamide}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & -0.04 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & -0.04 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/acetone_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:acetone_overlaps}
Overlap between ground and other calculated excited states for acetone}
\begin{tabular}{l | c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A_{2}$ & 
\hspace{2mm} $1^1B_{1}$ & 
\hspace{2mm} $2^1A_{1}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & -0.16 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & -0.16 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/adenine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:adenine_overlaps}
Overlap between ground and other calculated excited states for adenine}
\begin{tabular}{l | c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $2^1A'$ & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $3^1A'$ & 
\hspace{2mm} $2^1A^{\prime\prime}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.11 & -0.00 & -0.04 & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & 0.11 &  & 0.00 & 0.49 & 0.00 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & -0.00 & 0.00 &  & 0.00 & 0.49 \\ 
\hspace{0.0mm} $3^1A'$ & -0.04 & 0.49 & 0.00 &  & -0.00 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.00 & 0.00 & 0.49 & -0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/benzene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzene_overlaps}
Overlap between ground and other calculated excited states for benzene}
\begin{tabular}{l | c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{2u}$ & 
\hspace{2mm} $1^1B_{1u}$ & 
\hspace{2mm} $1^1E_{1u}$ & 
\hspace{2mm} $2^1E_{2g}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & -0.27 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.00 &  & 0.00 & 0.01 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.00 & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1E_{1u}$ & 0.00 & 0.01 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1E_{2g}$ & -0.27 & 0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/benzoquinone_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:benzoquinone_overlaps}
Overlap between ground and other calculated excited states for benzoquinone}
\begin{tabular}{l | c c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A_{u}$ & 
\hspace{2mm} $1^1B_{1g}$ & 
\hspace{2mm} $1^1B_{3g}$ & 
\hspace{2mm} $1^1B_{1u}$ & 
\hspace{2mm} $1^1B_{3u}$ & 
\hspace{2mm} $2^1B_{3g}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{3g}$ & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 & -0.15 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.00 & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & -0.00 & 0.00 & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1B_{3g}$ & 0.00 & 0.00 & 0.00 & -0.15 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/butadiene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:butadiene_overlaps}
Overlap between ground and other calculated excited states for butadiene}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.22 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 0.22 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/cyclopentadiene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopentadiene_overlaps}
Overlap between ground and other calculated excited states for cyclopentadiene}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{2}$ & 
\hspace{2mm} $2^1A_{1}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & -0.15 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & -0.15 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/cyclopropene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cyclopropene_overlaps}
Overlap between ground and other calculated excited states for cyclopropene}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{1}$ & 
\hspace{2mm} $1^1B_{2}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/cytosine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:cytosine_overlaps}
Overlap between ground and other calculated excited states for cytosine}
\begin{tabular}{l | c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $2^1A'$ & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $3^1A'$ & 
\hspace{2mm} $2^1A^{\prime\prime}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & -0.00 & 0.12 & -0.00 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & -0.00 &  & -0.00 & 0.07 \\ 
\hspace{0.0mm} $3^1A'$ & 0.12 & -0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & -0.00 & 0.07 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/formaldehyde_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formaldehyde_overlaps}
Overlap between ground and other calculated excited states for formaldehyde}
\begin{tabular}{l | c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $2^1A_{1}$ & 
\hspace{2mm} $1^1A_{2}$ & 
\hspace{2mm} $1^1B_{1}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.18 & 0.00 & -0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.18 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1}$ & -0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/formamide_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:formamide_overlaps}
Overlap between ground and other calculated excited states for formamide}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.09 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & 0.09 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/furan_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:furan_overlaps}
Overlap between ground and other calculated excited states for furan}
\begin{tabular}{l | c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{2}$ & 
\hspace{2mm} $2^1A_{1}$ & 
\hspace{2mm} $3^1A_{1}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & -0.09 & -0.02 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & -0.09 & 0.00 &  & 0.05 \\ 
\hspace{0.0mm} $3^1A_{1}$ & -0.02 & 0.00 & 0.05 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/hexatriene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:hexatriene_overlaps}
Overlap between ground and other calculated excited states for hexatriene}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{u}$ & 
\hspace{2mm} $2^1A_{g}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.29 \\ 
\hspace{0.0mm} $1^1B_{u}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{g}$ & 0.29 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/imidazole_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:imidazole_overlaps}
Overlap between ground and other calculated excited states for imidazole}
\begin{tabular}{l | c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ & 
\hspace{2mm} $3^1A'$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.26 & -0.04 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & -0.26 & 0.00 &  & 0.08 \\ 
\hspace{0.0mm} $3^1A'$ & -0.04 & 0.00 & 0.08 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/naphthalene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:naphthalene_overlaps}
Overlap between ground and other calculated excited states for naphthalene}
\begin{tabular}{l | c c c c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{3u}$ & 
\hspace{2mm} $1^1B_{2u}$ & 
\hspace{2mm} $2^1A_{g}$ & 
\hspace{2mm} $1^1B_{1g}$ & 
\hspace{2mm} $2^1B_{3u}$ & 
\hspace{2mm} $2^1B_{1g}$ & 
\hspace{2mm} $2^1B_{2u}$ & 
\hspace{2mm} $3^1A_{g}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & -0.00 & 0.00 & -0.08 & -0.00 & 0.00 & -0.00 & -0.00 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & -0.00 &  & 0.00 & -0.00 & 0.00 & -0.01 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.00 & 0.00 &  & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{g}$ & -0.08 & -0.00 & 0.00 &  & -0.00 & -0.00 & 0.00 & -0.00 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & -0.00 & 0.00 & -0.00 & -0.00 &  & -0.00 & -0.11 & 0.00 \\ 
\hspace{0.0mm} $2^1B_{3u}$ & 0.00 & -0.01 & 0.00 & -0.00 & -0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1B_{1g}$ & -0.00 & 0.00 & 0.00 & 0.00 & -0.11 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & -0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/norbornadiene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:norbornadiene_overlaps}
Overlap between ground and other calculated excited states for norbornadiene}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A_{2}$ & 
\hspace{2mm} $1^1B_{2}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/octatetraene_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:octatetraene_overlaps}
Overlap between ground and other calculated excited states for octatetraene}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{u}$ & 
\hspace{2mm} $2^1A_{g}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & -0.34 \\ 
\hspace{0.0mm} $1^1B_{u}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{g}$ & -0.34 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/propanamide_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:propanamide_overlaps}
Overlap between ground and other calculated excited states for propanamide}
\begin{tabular}{l | c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.04 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & 0.04 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/pyrazine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrazine_overlaps}
Overlap between ground and other calculated excited states for pyrazine}
\begin{tabular}{l | c c c c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{3u}$ & 
\hspace{2mm} $1^1B_{2u}$ & 
\hspace{2mm} $1^1A_{u}$ & 
\hspace{2mm} $1^1B_{2g}$ & 
\hspace{2mm} $1^1B_{1g}$ & 
\hspace{2mm} $1^1B_{1u}$ & 
\hspace{2mm} $2^1B_{2u}$ & 
\hspace{2mm} $2^1B_{1u}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 & -0.29 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 0.00 & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  & 0.00 & -0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1u}$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.01 \\ 
\hspace{0.0mm} $2^1B_{2u}$ & 0.00 & 0.00 & -0.29 & 0.00 & 0.00 & -0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1B_{1u}$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/pyridazine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridazine_overlaps}
Overlap between ground and other calculated excited states for pyridazine}
\begin{tabular}{l | c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{1}$ & 
\hspace{2mm} $1^1A_{2}$ & 
\hspace{2mm} $2^1A_{1}$ & 
\hspace{2mm} $2^1A_{2}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.03 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.00 &  & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.00 & 0.00 &  & 0.00 & 0.11 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.03 & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{2}$ & 0.00 & 0.00 & 0.11 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/pyridine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyridine_overlaps}
Overlap between ground and other calculated excited states for pyridine}
\begin{tabular}{l | c c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{2}$ & 
\hspace{2mm} $1^1B_{1}$ & 
\hspace{2mm} $1^1A_{2}$ & 
\hspace{2mm} $2^1A_{1}$ & 
\hspace{2mm} $3^1A_{1}$ & 
\hspace{2mm} $2^1B_{2}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & -0.04 & 0.11 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 & -0.31 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & -0.04 & 0.00 & 0.00 & 0.00 &  & -0.10 & 0.00 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 0.11 & 0.00 & 0.00 & 0.00 & -0.10 &  & 0.00 \\ 
\hspace{0.0mm} $2^1B_{2}$ & 0.00 & -0.31 & 0.00 & 0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/pyrimidine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrimidine_overlaps}
Overlap between ground and other calculated excited states for pyrimidine}
\begin{tabular}{l | c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{1}$ & 
\hspace{2mm} $1^1A_{2}$ & 
\hspace{2mm} $1^1B_{2}$ & 
\hspace{2mm} $2^1A_{1}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & 0.20 \\ 
\hspace{0.0mm} $1^1B_{1}$ & 0.00 &  & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{2}$ & 0.00 & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.20 & 0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/pyrrole_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:pyrrole_overlaps}
Overlap between ground and other calculated excited states for pyrrole}
\begin{tabular}{l | c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $2^1A_{1}$ & 
\hspace{2mm} $1^1B_{2}$ & 
\hspace{2mm} $3^1A_{1}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.02 & 0.00 & 0.01 \\ 
\hspace{0.0mm} $2^1A_{1}$ & 0.02 &  & 0.00 & -0.08 \\ 
\hspace{0.0mm} $1^1B_{2}$ & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $3^1A_{1}$ & 0.01 & -0.08 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/tetrazine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:tetrazine_overlaps}
Overlap between ground and other calculated excited states for tetrazine}
\begin{tabular}{l | c c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1B_{3u}$ & 
\hspace{2mm} $1^1A_{u}$ & 
\hspace{2mm} $1^1B_{2u}$ & 
\hspace{2mm} $1^1B_{1g}$ & 
\hspace{2mm} $2^1A_{u}$ & 
\hspace{2mm} $1^1B_{2g}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{3u}$ & 0.00 &  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{u}$ & 0.00 & 0.00 &  & 0.00 & 0.00 & -0.22 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2u}$ & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1B_{1g}$ & 0.00 & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A_{u}$ & 0.00 & 0.00 & -0.22 & 0.00 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $1^1B_{2g}$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/thymine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:thymine_overlaps}
Overlap between ground and other calculated excited states for thymine}
\begin{tabular}{l | c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ & 
\hspace{2mm} $2^1A^{\prime\prime}$ & 
\hspace{2mm} $3^1A'$ & 
\hspace{2mm} $4^1A'$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & -0.00 & 0.00 & -0.29 & 0.12 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.00 &  & 0.00 & -0.01 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & -0.00 & -0.01 &  & 0.00 & 0.31 & -0.26 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.00 \\ 
\hspace{0.0mm} $3^1A'$ & -0.29 & 0.00 & 0.31 & 0.00 &  & -0.67 \\ 
\hspace{0.0mm} $4^1A'$ & 0.12 & 0.00 & -0.26 & 0.00 & -0.67 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/triazine_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:triazine_overlaps}
Overlap between ground and other calculated excited states for triazine}
\begin{tabular}{l | c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A_{1}^{\prime\prime}$ & 
\hspace{2mm} $1^1A_{2}^{\prime\prime}$ & 
\hspace{2mm} $1^1E^{\prime\prime}$ & 
\hspace{2mm} $1^1A_2^\prime$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{1}^{\prime\prime}$ & 0.00 &  & 0.00 & -0.00 & 0.00 \\ 
\hspace{0.0mm} $1^1A_{2}^{\prime\prime}$ & 0.00 & 0.00 &  & -0.08 & 0.00 \\ 
\hspace{0.0mm} $1^1E^{\prime\prime}$ & 0.00 & -0.00 & -0.08 &  & 0.00 \\ 
\hspace{0.0mm} $1^1A_2^\prime$ & 0.00 & 0.00 & 0.00 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 


==> overlaps-needs to be double checked/uracil_overlaps.tex <==
\begin{table}[htp]
\caption{ 
\label{tab:uracil_overlaps}
Overlap between ground and other calculated excited states for uracil}
\begin{tabular}{l | c c c c c c c}
\hline\hline
\hspace{2mm} & 
\hspace{2mm} Ground State & 
\hspace{2mm} $1^1A^{\prime\prime}$ & 
\hspace{2mm} $2^1A'$ & 
\hspace{2mm} $2^1A^{\prime\prime}$ & 
\hspace{2mm} $3^1A'$ & 
\hspace{2mm} $4^1A'$ & 
\hspace{2mm} $3^1A^{\prime\prime}$ 
\\[2pt] 
\hline 
\hspace{0.0mm} Ground state &  & 0.00 & 0.07 & 0.00 & 0.18 & 0.00 \\ 
\hspace{0.0mm} $1^1A^{\prime\prime}$ & 0.00 &  & -0.00 & 0.00 & 0.00 & 0.00 \\ 
\hspace{0.0mm} $2^1A'$ & 0.07 & -0.00 &  & 0.00 & -0.04 & 0.00 \\ 
\hspace{0.0mm} $2^1A^{\prime\prime}$ & 0.00 & 0.00 & 0.00 &  & 0.00 & 0.04 \\ 
\hspace{0.0mm} $4^1A'$ & 0.18 & 0.00 & -0.04 & 0.00 &  & 0.00 \\ 
\hspace{0.0mm} $3^1A^{\prime\prime}$ & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 &  \\ 
\hline\hline 
\end{tabular} 
\end{table} 

